ASPaeroFlow: Decomposition Heuristics for Joint Air Traffic Flow & Capacity Management

While mathematical models act as vital decision support systems for operational Air Traffic Flow and Capacity Management (ATFCM), existing approaches isolate Air Traffic Flow Management (ATFM) from Dynamic Airspace Configuration (DAC). This separation introduces an unresolved circular dependency between fixed-demand and fixed-capacity assumptions. Although joint optimization resolves this gap, the enlarged search space renders exact models computationally intractable for medium- to large-scale instances. To bridge this gap, we propose ASPaeroFlow: a heuristic for the joint ATFCM; it combines instance-space decomposition heuristics with a local exact approach using Answer Set Programming. We benchmark ASPaeroFlow from small to industry-sized instances and compare it with exact and alternative approaches. The results indicate that (1) the heuristic provides a computational middle ground between exact methods and operational baselines; (2) simultaneous optimization can outperform sequential optimization on joint ATFCM; and (3) an ablation study indicates that DAC has a larger impact on solution quality than flow measures.

==> 20260607_OLD_RELATED_WORK.tex <==
% I REALLY LIKE THIS RELATED WORK SECTION BUT TOO SPACY:
\noindent
\textbf{Related Work}.
Dynamic Airspace Configuration (DAC) and Dynamic Airspace Sectorization (DAS) aim to design airspace to use available resources optimally.
DAC constructs airspace, by combining basic building blocks, whereas DAS partitions airspace freely into sectors~\cite{lui_robust_2025}.
Our approach constructs sectors from atomic blocks, where the sectors partition the overall airspace.
Although ASPaeroFlow integrates ideas from both DAC and DAS, ASPaeroFlow leans more towards DAC and therefore use DAC henceforth.
%
Heuristics for sector design exist:
sectors should be connected and ideally convex; flights should remain in a sector for a minimum amount of time; a flight should never re-enter a sector~\cite{sergeeva_3d_2015}.
Automatic sector design aims at designing appropriate sectors with methods ranging from genetic algorithms and Voronoi cells~\cite{sergeeva_3d_2015, yin_multi-objective_2016, xue_airspace_nodate,chandra_integration_2024},
approaches spanning the timeline from strategic to the tactical level~\cite{romero_smarts_nodate},
graph-based approaches~\cite{feng_graphdac_2023}, %,chen_dynamic_2014},
machine learning~\cite{xu_dynamic_2024}, or mixed integer programming and groupings of sectors~\cite{lui_airspace_2024}.
We generate connected sectors on the graph level.

Flow optimization aims at routing network flow (aircraft) optimally, while adhering to side constraints.
A current challenge is to move from the \emph{Computer Assisted Slot Allocation} (CASA) algorithm used in Europe, to more efficient methods.
CASA resolves overloaded sectors, by assigning flights to slots - and thereby effectively delaying them - according to the ``First Planned - First Served'' principle~\cite{eurocontrol_experimental_centre_innovative_2001,bucuroiu_european_2025}.
Research into ATFM investigated the optimization of delaying and reroutings~\cite{bertsimas_air_2008}, where it was shown that the restriction to delaying is already $NP$-hard~\cite{bertsimas_air_1998}.
Recent work explores notions of fairness for airlines~\cite{bertsimas2016fairness}, lexicographic optimization~\cite{dalmau_multi-objective_2024}, or
improvements of computational aspects~\cite{berstimas_ATFM_2011,bolic_reducing_2017,balakrishnan_optimal_nodate}.
Heuristics are used where exact methods run into computational bottleneck~\cite{dal_sasso_planning_2019}.
Survey papers for ATF(C)M exist~\cite{ng_review_2018,degas_survey_2022,aditya_review_2024}. %,chen_recent_2024}.
However, only a few methods enable the integration of DAC into ATFM, which model DAC as a fixed input to the flow optimization~\cite{agustin_air_2012,garcia-heredia_combinatorial_2019},
where to the best of our knowledge no method allows for sequential or simultaneous joint optimization.

Methodologically, Answer Set Programming (ASP) has been used in industrial projects where a balance between efficiency and interpretability was deemed necessary.
Examples include projects on product configuration~\cite{balazova_smart_2025,comploi-taupe_interactive_nodate} or train scheduling~\cite{abels_train_2021}.
Regarding aviation, proposals for the usage of ASP for efficient drone scheduling~\cite{nguyen_optimized_2024} or optimization for mission schedules on vertiports~\cite{kim_enhancing_2025} exist.
%
We investigate the usage of ASP in ATFCM research, as it is a promising symbolic-AI based approach and enables the future integration of explainability features, 
which sets ourselves apart from many papers in ATFCM focusing on MIP.
One of the main limiting factors of ASP for industrial use-cases is the so-called \emph{grounding bottleneck}, which is a combinatorial explosion in the variable replacement step~\cite{semmelrock_investigating_2025,BEISER_WOLTRAN_HECHER_2025}.
%
To enable scalability, we integrate ASP in a construction heuristics based on problem decomposition~\cite{el-kholany_problem_2022}.




\vspace{-0.2cm}
\section{Preliminaries}
\label{sec:preliminaries}
\vspace{-0.2cm}

\noindent
\textbf{Graph Theory}.
We assume basic familiarity with graph theory;
normally, we use weighted undirected finite simple graphs $G = (V,E)$.
Let $P$ be the set of \emph{simple} paths.
For $p \in P$, let $\textit{weight}(p)$ be the weighted length of $p$.
A trajectory $\textit{tr}$ is a path $p \in P$ augmented with timestamps.
For $v_i \in p$, $\textit{tr}$ contains a pair $(v_i,t_i)$ with strictly increasing times $t_i < t_{i+1}$.
%
We consider Euclidean and geodesic graphs.
Euclidean graphs define the distance between two vertices $v_i, v_j \in V$ as the Euclidean norm: $d(v_i, v_j) = ||v_i - v_j||_2$.
Geodesic graphs define the distance $d(v_i,v_j)$ as the great circle distance.





==> 20260616_OLD_DATA_GENERATOR.tex <==
\section{Data Generator}
\label{sec:data-generator}


  \begin{figure}[t]
      \centering
      \begin{subfigure}[t]{0.45\textwidth}
          \includegraphics[width=0.99\textwidth]{00_SUBMISSION/imgs/schematics/navgraph_schematics.pdf}
          \caption{
            Navpoints are connected by edges, while the sectors are drawn as Voronoi cells.
            %Country borders are in dark-gray and airports as green squares.
            %Flights follow routes on the navpoint graph through sectors.
          }
        \end{subfigure}
        \begin{subfigure}[t]{0.45\textwidth}
          \includegraphics[width=0.99\textwidth]{00_SUBMISSION/imgs/overload_maps/central_europe_overaload.pdf}
          \caption{
            Aggregated routes and overload for the instance before optimization.
            %(initial static configuration).
            %Aggregated routes are shown in blue.
            %Aggregated overload (demand greater than capacity) is shown in red.
            %Filed flight routes are aggregated over the instance and shown in blue.
            %Demand is aggregated over time for an assumed initial static sector configuration and shown in red.
          }
        \end{subfigure}
        \begin{subfigure}[t]{0.08\textwidth}
          \includegraphics[width=0.8\textwidth]{00_SUBMISSION/imgs/overload_maps/central_europe_overaload_legends.pdf}
        \end{subfigure}
        \vspace{-0.3cm}
        \caption{
        Figure displaying an instance of CE (Central Europe), from the data generator.
        %Geographically, the instance shows the 2D-projected navpoint structure of central Europe, with a focus on Austria.
        %The graph was generated using the Gabriel criterion with a maximum edge length of 100 km.
        %Sectors are generated connected with a default sector size of $30$ navpoints.
        %We generated $31,622$ flights with a time granularity of $60$ ($1$ minute timesteps).
        }
      \label{fig:schematic-general-graph}
      \vspace{-0.5cm}
  \end{figure}
%
Data in ATM research is often closed source, due to privacy concerns or the fear of competitive disadvantage.
Although these concerns are understandable from an economic perspective, they are disadvantageous for science -- which leads to two common issues:
(a) published research cannot be reproduced, thereby manifesting itself in a so-called reproducibility crisis;
(b) researchers relying on open data are sometimes forced to use datasets that are ill-suited to the task.
In order to circumvent this problem, movements have been initiated, such as the formation of the Open Science Alliance for ATM research~\cite{bolic_roadmap_2024}.
However, open data for ATFCM research is still scarce.
This paper takes a pro-open-data stance, by extending a data generator built from publicly available open data, which is then used to verify the implementation of the heuristics.
While a previous version of the data generator provided the basic ability to generate realistic flight data, we extend it to generate realistic navpoint data; previously only grid-graphs were available.
The data generator is available on GitHub\footnote{GitHub Link: \url{https://github.com/alexl4123/ASPaeroFlow-DataGenerator}}. 
We briefly describe its workings and our extension and see Figure~\ref{fig:schematic-general-graph} for an example.
%
%
\vspace{-0.5cm}
%\smallskip
%\noindent
%\subparagraph*{Navpoint Data Generation.}
\subparagraph{Navpoint Data Generation.}
%
Our updated graph generator supports now two modes: (1) real-world navpoint and airport data, or (2) grid-graph navpoint and real-world airport data.
For our geographic data, we use \texttt{OurAirports-Data}\footnote{\url{https://github.com/davidmegginson/ourairports-data}}, licensed under \texttt{The Unlicense}, and \texttt{BlueSky}~\cite{hoekstra_bluesky_2016} data under the \texttt{GNU General Public License}, originally taken from the X-Plane simulator.
Combining the fixes and navpoint data from BlueSky and the airport data from OurAirports leads to a graph with $\approx 160,000$ navpoints.
The generator provides options to include various filter options, like minimum separation of navpoints, different edge connection structures (Gabriel graph, local cliques), or specification of altitudes.
%
%\smallskip
%\noindent
\vspace{-0.5cm}
%\subparagraph*{Flight Data-Pair Generation.}
\subparagraph{Flight Data Generation.}
%
The flight-pair generation is performed from a probabilistic model of departure and destination counts, which is built upon the COVID-19 dataset of the \textit{OpenSky Network}~\cite{strohmeier_crowdsourced_2021}.
%The OpenSky network collects and stores live aviation surveillance data.
%The COVID-19 dataset is licensed under \texttt{CC-BY} and spans January 2019 to December 2021.
We generate flights using a Poisson model, where airports have a sending strength comparable to the number of departures per airports in a user-specified time-bin.
The arrival airport is computed in a second step, by a discrete probability distribution which models the origin-destination pairs for a given time-bin.
%
Trajectories are generated based on shortest origin-destination pairs on the navpoint graph.
Multi-leg flights are generated iteratively by available aircraft counts at an airport.
Sectors are generated by a breadth-first search algorithm that ensures connected sectors.

